Video Capsule Endoscopy Classification using Focal Modulation Guided Convolutional Neural Network

Video capsule endoscopy is a hot topic in computer vision and medicine. Deep learning can have a positive impact on the future of video capsule endoscopy technology. It can improve the anomaly detection rate, reduce physicians' time for screening, and aid in real-world clinical analysis. CADx classification system for video capsule endoscopy has shown a great promise for further improvement. For example, detection of cancerous polyp and bleeding can lead to swift medical response and improve the survival rate of the patients. To this end, an automated CADx system must have high throughput and decent accuracy. In this paper, we propose FocalConvNet, a focal modulation network integrated with lightweight convolutional layers for the classification of small bowel anatomical landmarks and luminal findings. FocalConvNet leverages focal modulation to attain global context and allows global-local spatial interactions throughout the forward pass. Moreover, the convolutional block with its intrinsic inductive/learning bias and capacity to extract hierarchical features allows our FocalConvNet to achieve favourable results with high throughput. We compare our FocalConvNet with other SOTA on Kvasir-Capsule, a large-scale VCE dataset with 44,228 frames with 13 classes of different anomalies. Our proposed method achieves the weighted F1-score, recall and MCC} of 0.6734, 0.6373 and 0.2974, respectively outperforming other SOTA methodologies. Furthermore, we report the highest throughput of 148.02 images/second rate to establish the potential of FocalConvNet in a real-time clinical environment. The code of the proposed FocalConvNet is available at https://github.com/NoviceMAn-prog/FocalConvNet.

==> takeout.tex <==
Bodenstedt et al.~\cite{bodenstedt2018comparative} organized "EndoVis 2015 Instrument sub-challenge" for developing new techniques and benchmarking the \ac{ML} algorithm for segmentation and tracking of the instruments on common dataset. The organizers challenged on two different tasks, (1) Segmentation, (2) Tracking. The goal of the challenge was to address the problem related to segmentation and tracking of articulated instruments in both laparoscopic and robotic surgery\footnote{\url{https://endovissub-instrument.grand-challenge.org/EndoVisSub-Instrument/}}. A comprehensive evaluation of the methods used in instrument segmentation and tracking task for minimally invasive surgery is summarized in this work~\cite{bodenstedt2018comparative}. The extensive results evaluation showed that modern deep learning was a better choice for instrument segmentation and tracking task. 

In 2017, a follow up to the previous 2015 challenge was organized called "Robotic Instrument Segmentation Sub-Challenge"\footnote{\url{https://endovissub2017-roboticinstrumentsegmentation.grand-challenge.org/}}. The challenge was part of Endoscopic vision challenge was organized at \ac{MICCAI} 2017. This challenge offered three tasks: (1) Binary segmentation task, (2) Parts based segmentation task, and (3) Instrument type segmentation task. The goal of the binary segmentation task was to separate the image into an instrument and background. Parts segmentation challenged the participants to divide the binary instrument into a shaft, wrist, and jaws. Type Segmentation challenged the participants to identify different instrument types. A detailed description of the challenge task, dataset, methodologies used by ten participating teams in different tasks, challenge design, and limitation of the challenge can be found in the challenge summary paper~\cite{allan20192017}. 


In 2019, a similar Challenge called "Robust Medical Instrument Segmentation Challenge 2019"\footnote{\url{https://robustmis2019.grand-challenge.org/}} was organized by Roß et al.~\cite{ross2020robust}. This challenge offered three tasks (1) Binary segmentation, (2) Multiple instance detection, and (3) Multiple instance segmentation. The challenge was focused on addressing two key issues in surgical instruments, \textit{Robustness} and \textit{Generalization}, and benchmark medical instrument segmentation and detection on the provided surgical instrument dataset. We participated in the binary segmentation task of the challenge. In this paper, we present our approach used for binary segmentation tasks for endoscopic instrument segmentation. 

%They used eight-fold cross-validation, where seven-fold were used for training, and one fold was used for testing. 



%Kalavakonda et al. \cite{kalavakonda2019autonomous} evaluated three deep learning architectures for binary segmentation. All the architecture was based on the encoder-decoder network. The first architecture was based on the Vanilla U-Net~\cite{ronneberger2015u}, and the other two were based on the transfer learning mechanism. 

In addition to these challenges, there are works on instrument segmentation in robot-assisted surgery~\cite{shvets2018automatic,pakhomov2019deep}, neurosurgical instrument segmentation~\cite{kalavakonda2019autonomous}, surgical instrument segmentation on minimally-invasive robot-assisted procedures~\cite{azqueta2019segmentation}, instrument tracking~\cite{laina2017concurrent}, and endoscopic instrument segmentation~\cite{isensee2020or}. 



%The learning rate for the optimizer is set to 1e-4. We prefer a lower learning rate, as it makes sure that the model parameters are updated slowly and carefully. We reduce the learning rate by a factor of 0.1 when the validation loss does not decrease in $10$ consecutive epochs, this improves our performance a lot.  We have also used early stopping to keep the model from overfitting, which is a good practice.

%We have implemented the proposed architecture using the Keras framework~\cite{chollet2015keras} with TensorFlow~\cite{abadi2016tensorflow} as backend running on the Experimental Infrastructure for Exploration of Exascale Computing (eX3), NVIDIA DGX-2 machine. As the model is having very low trainable parameters, we can set batch size up to 128, but we have chosen to use 64 in our case. We have resized the dataset from 540 x 960 pixels to 56 x 512 pixels for better utilization of the GPU and it also helps in reducing the training time. We have trained our model on 200 epochs with Nadam optimizer and dice coefficient as the loss function. The learning rate for the optimizer is set to 1e-4. We prefer a lower learning rate, as it makes sure that the model parameters are updated slowly and carefully. We reduce the learning rate by a factor of 0.1 when the validation loss does not decrease in $10$ consecutive epochs, this improves our performance a lot.  We have also used early stopping to keep the model from overfitting, which is a good practice.




New paper


% It can play a crucial role in full instrument pose estimation and improve user interaction with the robotic system.

% However, both accurate and real-time segmentation of surgical instruments in endoscopy is still a challenging issue.


% The major challenges remain in designing a lightweight deep learning model with low computational cost and high speed to be integrated with the endoscopic hardware devices to be deployed for the clinical settings.

% We propose an automated semantic segmentation architecture called NanoNet, a novel architecture for instrument segmentation in endoscopy to address this challenge.

% The main aim of the task to classify each surgical instrument's pixel into either a background class or instrument class.

% Experiments demonstrate our superior trade-off among lightweight, speed, computation, parameter use, and performance metrics.

% NanoNet achieves a dice similarity coefficient of ... and inference speed of .....which is the state-of-the-art on 2017 MICCAI EndoVis Robotic Instrument Segmentation Challenge dataset, Kvasir-SEG and Robust Medical Instrument Segmentation challenge dataset.

% Moreover, the model size is very small with only 36000 parameters. Despite of the tiny model size, the NanoNet achieves promising results. 


\ac{VCE} is a technology for capturing the video  inside the \ac{GI} tract.  It remains the first choice for screening of small bowel diseases~\cite{}. 


\acf{MIS} and robot-assisted surgery is a new field of research. In the recent years, minimally invasive surgery, computer and robotic-assisted intervention have attracted significant attention in surgical practice. \ac{MIS} is a procedure that has less or negligible cuts, less pain, and shorter hospital stay and fewer complications as compared to traditional laparoscopic surgery. \ac{MIS} gaining increasing level of trust from surgeon. Therefore, it has improved the traditional surgical procedure and help to overcome the limitations of traditional laparoscopic surgery~\cite{azqueta2020segmentation}. However, manipulation of the surgical instrument in limited restricted operating space causes problem such as limited field of view of the endoscope, reduce in surgeon's dexterity, and lacks perception of force feedback~\cite{qiu2019real}. 





Endoscopy is the technique for looking inside the body using an endoscope. 
Endoscopy (Upper \ac{GI} endoscopy) is the procedure performed by gastroenterologists who uses the endoscope to diagnose and treat the problem of the upper digestive system. Upper \ac{GI} tract includes upper part of digestive system such as esophagus, stomach and duodenum. Upper \ac{GI} endoscope can help to diagnose the conditions such as difficulty in swallowing, abdominal pain, bleeding, ulcer, and tumor. In some cases it might be necessary to take biopsy for later examination under microscope. The endoscope can be used to treat a problem such as active bleeding from ulcer. 






























































% \begin{table*}[t!]
% \footnotesize
% \def\arraystretch{1.1}
% \caption{Available instrument datasets}
% \label{tab:availabledataset}
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \toprule
% \textbf{Dataset} & \textbf{Content} & \textbf{Resolution} & \textbf{Size} &  \textbf{Task type} & \textbf{Procedure}  & \textbf{Available} \\ \midrule

% % \begin{tabular}[c]{@{}l@{}}Instrument segmentation\\ and tracking (2015)~\cite{bodenstedt2018comparative}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Rigid and robotic\\ instruments\end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Segmentation \\ and tracking\end{tabular} & Laparoscopy \\ \hline

% % \begin{tabular}[c]{@{}l@{}}Robotic Instrument \\ Segmentation (2017)~\cite{allan20192017}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Robotic surgical\\  instruments\end{tabular}  & & & & \begin{tabular}[c]{@{}l@{}}Binary segmentation,\\ part based segmentation, \\instrument segmentation\end{tabular} & 

% % \begin{tabular}[c]{@{}l@{}}Abdominal\\ porcine  \end{tabular}  \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Robotic Scene\\ Segmentation (2018)~\cite{allan20192018}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Surgical instruments\\ and other  \end{tabular}& & & & \begin{tabular}[c]{@{}l@{}}Multi-instance\\  segmentation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Robotic\\ nephrectomy  \end{tabular} \\ \hline

% \begin{tabular}[c]{@{}l@{}}Robust Medical instrument\\ segmentation (2019)~\cite{ross2020robust}\end{tabular} & \begin{tabular}[c]{@{}l@{}} laparoscopic\\ instrument \end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Binary  segmentation, \\ multiple instance\\ detection,  multiple  \\ instance segmentation\end{tabular} & Laparoscopy \\ \hline

% Kvasir-Instrument~\cite{jha2020kvasir} & \begin{tabular}[c]{@{}l@{}} Diagnostic and\\ therapeutic tools\\ in endoscopic images\end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Binary segmentation\\ Detection and localization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gastroscopy\\  \& colonoscopy\end{tabular} \\ \bottomrule
% \end{tabular}
% \end{table*}



% \begin{table*}[!t]
% \centering
% \caption{Result on ISIC 2018 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method}  & \textbf{Backbone} & \textbf{Parameters} & \textbf{DSC}  & \textbf{mIoU}  & \textbf{Recall} & \textbf{Precision} & \textbf{F2-score}  & \textbf{Overall Acc} & \textbf{FPS} \\ \midrule

% NanoNet-A && 235,425  & 0.8651 & 0.8384 & 0.8517 & 0.9084  & & & \\ \hline
% NanoNet-B && 132,049 & 0.8685 & 0.8381 & 0.8629 & 0.9002   & & & \\ \hline
% NanoNet-C&& 36,561 & 0.8601 & 0.8322 & 0.8645 & 0.8831  & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \begin{table}[!t]
% \caption{Result on the binary segmentation task of 2017 Robotic Instrument segmentation challenge}
% \def\arraystretch{1.2}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Method & Parameters & Dice   & mIoU   & Recall & Precision \\ \hline
% NanoNet-A & 235,425  & 0.0000 & 0.0000 & 0.0000 & 0.0000    \\ \hline
% NanoNet-B & 132,049 & 0.0000 & 0.0000 & 0.0000 & 0.0000   \\ \hline
% NanoNet-C & 36,561 & 0.0000 & 0.0000 &0.0000 & 0.0000    \\ \hline
% \end{tabular}
% \label{tab:result}
% \end{table}

%We have evaluated NanonNet using four instrument segmentation benchmarks. The experiments demonstrates state-of-the-art speed and superior performance with all on all four datasets.
%Our main goal was to develop an efficient algorithms that requires low computational and memory requirements. 

% The dataset contains two folders i.e, Prokto and Rectum. These are two different types of procedures. These folders contain $8$ sub-folders inside them, which represents $8$ different types of surgeries. Each of these sub-folders itself contains multiple sub-folders which contains the images and their respective masks. From these $8$ sub-folders, we use $6$ sub-folders for training, $1$ sub-folder for validation and $1$ sub-folder testing. 

% We train the model using the image dataset. The sample of the training dataset and their corresponding masks can be found in the first and second column of Figure~\ref{fig:results2}. The original size of the images is 960$\times$540. We split the dataset using 80\% of dataset for training and remaining 20\% for the validation (evaluation). The training dataset was augmented and resized. We performed augmentation such as center crop, random crop, horizontal flip, vertical flip, scale augmentation, cutout, and gray-scale. The validation dataset is not augmented and is directly resized into 512$\times$256. 

%There are numerous computer vision based approaches developed for instrument segmentation~\cite{shvets2018automatic,ni2019attention}.

%Semantic segmentation is an important task in the field of computer vision. It is the task of labeling each pixel in an image with a class label that helps to distinguish different objects in an image. It can also help in improving robotics-assisted surgery by enabling the identification and precise localization of surgical instruments from the background tissue in the endoscopic images. 

% (https://arxiv.org/pdf/2006.02706v1.pdf). 
%Therefore, an accurate semantic segmentation would provide information regarding the presence of multiple instruments in the videos or images. %Many algorithms for segmentation, tracking, and detection have been proposed in the literature, however the problem of real-time semantic segmentation still remains challenge. 

%TOOD:Nikhil

% The architecture of the NanoNet follows an encoder-decoder approach as shown in figure 1. The proposed architecture uses a pre-trained MobileNetV2 model trained on the ImageNet dataset as an encoder.

%\subsubsection{Kvasir-SEG}
%\subsubsection{ISIC 2018}

% Now the concatenated feature maps pass through the modified residual block, which further increases the generalization capacity of the decoder. The output from the modified residual block is concatenated with the 3 x 3 standard convolution with the only one feature channel and a sigmoid activation. After the feature maps pass through all the four decoder block, the output of the last decoder block is fed to a 3 x 3 standard convolution which is followed by the sigmoid activation. Finally, the sigmoid activation function gives us the binary segmentation map.

% In our modified residual block, we replace the two $3\times3$ standard convolution with depth-wise separable convolution, which helps us in drastically reducing the number of parameters of the proposed architecture.

% The input image is first fed into the pre-trained MobileNetV2 encoder, after that the encoder output goes into the a modified residual block after which it is followed by a sequence decoder blocks. The decoder block uses a bilinear upsampling to increase the spatial dimension (height and width) of the input feature maps. After that, it is concatenated with the appropriate feature maps from the pre-trained encoder using the skip connection. Now the concatenated feature maps pass through the modified residual block and then the output of the modified residual block is concatenated with the 3 x 3 standard convolution with the only one feature channel. After the feature maps pass through all the four decoder block, the output of the last decoder block is fed to a 3 x 3 standard convolution which is followed by the sigmoid activation. Finally, the sigmoid activation function gives us the binary segmentation map.



% \begin{table*}[!t]
% \centering
% \caption{Result on EAD 2019 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ \hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ \hline
% NanoNet-A & MobileNetV2 & & &  & & & & &  \\ \hline
% NanoNet-B &MobileNetV2 &  & & &  & & & & \\ \hline
% NanoNet-C &MobileNetV2 & &  &  &  & & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \begin{table*}[!t]
% \centering
% \caption{Result on Endocv2020 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ \hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ \hline
% NanoNet-A & MobileNetV2 & & &  & & & & &  \\ \hline
% NanoNet-B &MobileNetV2 &  & & &  & & & & \\ \hline
% NanoNet-C &MobileNetV2 & &  &  &  & & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}






% \begin{table*}[!t]
% \scriptsize
% \centering
% \caption{Result on 2019 CaDIS dataset}
% \footnotesize
% \begin{tabular}{l|l|l|l|l|l|l|l|l| l}
% \toprule
% \textbf{Method} & \textbf{Backbone} & \textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision} & \textbf{F2} & \textbf{Overall acc} & \textbf{FPS} \\ \midrule

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ %\hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ %\hline
% NanoNet-A &MobileNetV2 &235,425 & & & & & & & \\ %\hline
% NanoNet-B &MobileNetV2 &132,049  & & & & & & & \\ %\hline
% NanoNet-C &MobileNetV2 &36,561  & & & & & & & \\


% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}




% \subsection{Ablation Study on Kvasir-Instrument}
% \subsection{Ablation Study on Robust-MIS}
% \subsection{Ablation Study for FCB}
% \subsection{Ablation Study for FCB}


%===========================================================================

% \begin{table*}[!t]
% \scriptsize
% \centering
% \caption{Result on 2019 ROBUST-MIS dataset}
% \footnotesize
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline
% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ %\hline
% ResUNet~\cite{zhang2018road}& &- & & & & & & & \\ %\hline
% NanoNet-A &MobileNetV2 &235,425 &0.7248 &0.6701 &0.7333 &0.8806 &0.8545 &0.9898 &22.00 \\ 
% NanoNet-B &MobileNetV2 &132,049 &0.7195 &0.6621 &0.7221 &0.8856 &0.8545 &0.9898 &25.60 \\ 
% NanoNet-C &MobileNetV2 &36,561  &0.7036 &0.6402 &0.7082 &0.8394 &0.8033 &0.9864 &26.34 \\
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \subsection{Evaluation Metrics}
% \label{sec:evaluationmetrics}
%For the evaluation of our model, we have chosen standard computer vision metrics such as Sørensen–dice coefficient (DSC), \ac{mIoU}, Precision, and Recall, Specificity, Accuracy and \ac{FPS}. 

% \begin{equation}{\label{eq:1}}
% \text{DSC (A,B)} = \frac{2 \times TP} {2 \times TP + FP + FN}
% \end{equation}
% %
% \begin{equation}
% \text{IoU (A,B)} = \frac{TP} {TP + FP + FN}
% \end{equation}
% %
% \begin{equation}{\label{eq:1}}
% \text{Recall}~(r) = \frac{TP} {TP + FN}
% \end{equation}
% %
% \begin{equation}{\label{eq:3}}
% \text{Precision}~(p) =\frac{TP} {TP + FP}
% \end{equation}
% %
% \begin{equation}{\label{eq:5}}
% \text{F2} = \frac{5p \times r} {4p + r}
% \end{equation}
% %
% \begin{equation}{\label{eq:6}}
% \text{Overall accuracy}~(Acc.) ={\frac{TP + TN} {TN + TN + FP + FP}} 
% \end{equation}
% %
% \begin{equation}{\label{eq:7}}
% \text {Frame Per Second}~(FPS) = {\frac{1} {sec /frame}}
% \end{equation}

% In the above equations, \textit{TP}, \textit{FP}, \textit{TN}, \textit{FN} represents true positives, false positives, true negatives, and false negatives, respectively, for the classification outputs. Based on these metrics, we will evaluate and compare the performance of our method. 




% \subsubsection{Robust-MIS Dataset}
% The first dataset used in the study is from the Robust Medical Instrument Segmentation (ROBUST-MIS)\footnote{\scriptsize \url{https://robustmis2019.grand-challenge.org}}. Heidelberg Colorectal (HeiCo) data set~\cite{maier2020heidelberg} includes a total of $5983$ images with their respective manually annotated masks. These training images are obtained from $16$ different surgeries with the two different types of procedures (Prokto and Rectum, $8$ surgeries each). The prokto consists of $2943$ images, and the rectum contains $3040$ images. The challenge also offers a video dataset. However, we have not used a video dataset for our experimental setup. 

% \subsubsection{Endovis Robotic Instrument segmentation Challenge dataset}
% The dataset is taken from the "Robotic Instrument Segmentation challenge" held at the 2017 MICCAI Endovis Challenge. The video frames are acquired from a da Vinci Xi robot. These images are from various porcine procedures. The dataset consists of 3000 images, out of which 1800 images were used for training, and 1200 images were used for testing. The images have a resolution of $1280\times1024$. There are seven types of surgical instruments in Endovis 2017. More details about the challenge and challenge dataset can be found from here \footnote{\scriptsize {\url{https://endovissub2017-roboticinstrumentsegmentation.grand-challenge.org/}}


%The paper is organized as follows. Section \ref{sec:relatedwork} describes the related work on instrument segmentation and highlights the need for real-time segmentation. Section \ref{sec:methods} describes the NanoNet architectures used in our study. Section \ref{sec:materials used} describes the material used to validate the proposed method. Section \ref{sec:results} describes the results. Section \ref{sec:Discussion} describes the discussion. Section \ref{sec:conclusion} describes the conclusion and highlights the future work. 


%This is an important contribution for vision-based minimal invasive surgery and can be useful for clinical trails.

%Moreover, we will investigate ways to optimize the network for achieving higher performance with the same number of parameters. We will work on detection and localization of the surgical instrument in near future. 



%Real-time segmentation of the endoscopy is a challenging problem. An automated pixel-wise segmentation of endoscopic images can reduce the risk for miss-detection. These applications can reduce the doctors' burden, improve the overall performance and clinical workflow. The semantic segmentation of medical images (colonosopic images) are challenging as compared to the segmentation of the natural images. It is challenging due to variation in lighting, shadows, the overlap between the instrument, reflection, occlusions from blood, fogging, or interference from the surgeon in the frame~\cite{bouget2017vision}. These challenges presence makes it difficult to distinguish between the polyp and background tissue. 

%\ac{MIS} gaining increasing level of trust from surgeon. Therefore, it has improved the traditional surgical procedure and help to overcome the limitations of traditional laparoscopic surgery~\cite{azqueta2020segmentation}.












%%%%%%new%%%%%%%%%%%%%%%%%%%%%%


%A lightweight model is preferred to be used in clinical settings. Moreover, the inference time of the Nanonet is real-time, and the model does not require any sort of initialization or post-processing, or temporal regularization, which can be considered as the strength of the work. 

%In the future, we plan to design an encoder from scratch, which can be even lighter than pre-trained MobilNetV2. We also plan to work with the medical experts to understand the images and procedure in-depth to group the segment and distinguish between semantically meaningful information. 
% In this paper, we proposed a novel lightweight architecture, NanoNet, designed for endoscopic image segmentation. The improved performance of the NanoNet is due to the use of a lightweight pre-trained MobileNetV2 model and modified residual block. The depthwise separable convolution is the main building block of the network because of which our model can achieve high performance with fewer trainable parameters. The experimental result on recent segmentation benchmarks on five endoscopy datasets demonstrates state-of-the-art speed and performance.  A lightweight model is preferred to be used in clinical settings. Moreover, the inference time of the Nanonet is real-time, and the model does not require any sort of initialization or post-processing, or temporal regularization, which can be considered as the strength of the work. In the future, we plan to design an encoder from scratch, which can be even lighter than pre-trained MobilNetV2. We also plan to work with the medical experts to understand the images and procedure in-depth to group the segment and distinguish between semantically meaningful information. 


%Chaurasia et al.~\cite{paszke2016enet} proposed efficient neural network (EDNet), that was especially designed for high accuracy and fast inference. The model was 18 times faster and requires less parameter providing similar accuracy on the CamVid, Cityscapes and SUN datasets. Garcia-Peraza-Herrera et al.~\cite{garcia2017toolnet} proposed two architectures, TOOLNetMS and ToolNetH that were trained end-to-end for real-time semantic segmentation of surgical tools. Yu et al.~\cite{yu2018bisenet} proposed bilateral segmentation network (BiSeNet) for improving the speed and accuracy for the real-time semantic segmentation. The model consists of spatial path and context path for preserving spatial information from the original images. This network makes the right balance between accuracy and speed on the CamVid, Cityscapes and SUN datasets. 


% \subsection{Dataset}
% \begin{figure}
%     \centering
%      \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/1.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/1_mask.png}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/2.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/2_masks.png} \\
%         \vspace{1mm}
%       \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/3.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/3_mask.png}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/4.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/4_mask.png}
%     \caption{Example dataset from Kvasir-Instrument}
%     \label{fig:kvasir-instrument}
% \end{figure}


% \subsection{Generalisability} 
% Generalization is the ability of the model to perform well on other institute datasets  or interventions.  To promote the generalization, we have tested our best methods trained on Kvasir-SEG with the CVC-ClinicDB dataset. The performance of the best detection, localisation, and segmentation methods have shown that the methods have good accuracy and generalization capabilities. However, the model's performance was not as good as they perform while trained and tested on the same dataset. This can be evidence by the quantitative and qualitative results (see Table~\ref{tab:resultEndotect2020,tab:resultMedico2020} and Figure~\ref{qualitativeresultsa}). This may be because two different images are captured using different endoscopic devices, making it difficult to generalize.


% \subsection{Kvasir-Instrument dataset}
% Kvasir-Instrument~\cite{jha2020kvasirInstrument} is publicly available datasets and consist of 590 frames from \ac{GI} endoscopy. These images are from various therapeutic or surgical procedures. These datasets are collected using standard endoscopic equipment from Olympus and Pentax. The dataset consists of original images, ground truth, and bounding box information. %The example of the dataset is shown in the Figure~\ref{fig:kvasir-instrument}. 


%We have curated a dataset for the generalizability test or domain adaptation test. Therefore, we train the model on the colonoscopy dataset and test it against the \ac{VCE} dataset.


% We only have the training dataset provided by the challenge organizers, so we use that dataset for training, validation and testing purpose. The dataset is obtained from two different procedures (Prokto and Rectum), each contain data for $8$ surgeries each. Out of these $8$ surgeries, we have used $6$ surgeries for training, $1$ for validation and $1$ for testing purpose. The original resolution of the images is $540 \times 960$. For our convenience, we resized all the images to $256\times512$.


%Despite the small model size, the NanoNet achieves competitive results, which is the major strength of the work. 

%Deep learning in gastrointestinal endoscopy has tremendous potential to improve clinical performance and assessment of patients. The semantic segmentation of an image can provide critical information during medical examinations, which can play a crucial role in patient safety. However, accurate and real-time segmentation of endoscopic images is still a challenging problem. The significant challenges remain in designing a lightweight deep learning model with low computational cost and high speed to be integrated with the endoscopic hardware devices to be deployed for the clinical settings. To improve the eminent problems in diagnosis endoscopy systems, we propose a novel automated architecture, NanoNet, for segmenting endoscopic images. Experimental results demonstrate that NanoNet achieves promising results for wireless capsule endoscopy, colonoscopy, tools, and surgical instrument images. Experiments show our superior trade-off among lightweight, speed, computation, parameter use, and performance metrics. Moreover, the model size is tiny, with only 36000 parameters. Despite the small model size, the NanoNet achieves promising results, which is the major strength of the work. 

%Convolutional neural networks can play a crucial role in assisting clinicians. There has been a significant progress in the area of medical image analysis, especially with the development of medical diagnosis support systems for assisting clinicians. Such systems can offer better medical diagnoses, which can positively impact the patient's health. However, the significant challenges remain within the availability of high-quality, diverse labeled medical datasets for experimentation to develop such clinically relevant systems.


%Upper \ac{GI} is consists of the esophagus, stomach, and duodenum. Endoscopy (Upper \ac{GI} endoscopy) is the procedure where gastroenterologists observe an internal organ inside the body using an endoscope. Upper \ac{GI}  endoscope helps diagnose the conditions such as bleeding, ulcer, tumor, abdominal pain, and trouble in swallowing. A biopsy is taken for further investigation in cases where gastroenterologists encounter suspicious tissue. Endoscopy is also useful for treatment (for example, active bleeding for ulcers).  

%In recent years, \ac{MIS}, computer and robotic-assisted intervention have attracted significant attention in surgical practice. It is a procedure that has fewer or minor cuts, less pain, and requires a shorter hospital stay and fewer complications as compared to traditional laparoscopic surgery. However, manipulation of the surgical instrument is limited, restricted operating space causes a problem such as limited field of view of the endoscope, reduction in surgeon's dexterity, and lacks the perception of force feedback~\cite{qiu2019real}.  

%Upper \ac{GI} consists of the esophagus, stomach, and duodenum. The lower \ac{GI} consists of the large intestine and anus. 






Deep learning in Video capsule endoscopy can aid clinical analysis and identify abnormalities in real world clinical application. Real-time investigation of endoscopy images is a practitioner-dependent and laborious procedure. Medical image classification methodologies have shown great promise in classification of anatomical structures, which in turn can be of great utility in identification of unwanted/deleterious structures. Timely detection of such elements for example, cancerous polyp and bleeding can lead swift medical response. To this extent, automated computer assisted detection systems must have high throughput along with decent accuracy. However real-time or instantaneous classification of frames procured using VCE is a challenging task. 


Recent advent of vision Transformers have advanced image classification in computer vision. In this paper, we propose \textit{FocalConvNet}, a focal modulation network integrated with lightweight convolutional layers for anatomical landmark classification. FocalConvNet leverages focal modulation to attain global context and allows global-local spatial interactions throughout the forward pass. Moreover, the convolutional block with it's intrinsic inductive/learning bias and capacity to extract hierarchical features allow our FocalConvNet to achieve favourable results with high throughput. We compare our FocalConvNet with other \ac{SOTA} on Kvasir-Capsule, a large-scale VCE dataset with 44,228 frames with 13 classes of different anomalies. Our proposed method achieves the weighted F1-Score, Recall and MCC of 0.6734, 0.6373 and 0.2974, respectively outperforming other \ac{SOTA} methodologies. Furthermore, we report the highest throughput of 148.02 images/second rate to establish the potential of FocalConvNet in a real-time clinical environment.


% A solution that makes it possible to conduct more efficient and large-scale screening is using VCEs. A VCE, also often called camera pill, is a small capsule type device (typically $11mm \times 25mm$), which can have an image sensor, bleeding sensor, pH-sensor, antenna, battery, light source and wireless transceiver. The pill is swallowed (fig 1.) to visualize the GI tract for subsequent diagnosis and detection of GI diseases. The VCEs have a resolution of around ($256 \times 256$), frame rates of 3-35 frames per second (adaptive frame rate with a feedback loop from the receiver and transmitter). They do not have optimum lightning, making it challenging to detect endoscopic findings in the captured images than in images from traditional endoscopes. Also, during VCE procedures, the intestine is not explained, unlike in conventional endoscopy, where the expansion allows for precise and non-obfuscated images of the intestine walls. Nevertheless, ongoing research focus at enhancing the VCEs’ hardware capabilities and at upgrading the techniques and algorithms developed for colonoscopies to work also for VCEs.  
    
     
% The multi-sensor VCE is swallowed to envision the GI tract for ensuing diagnosis and detection of GI tract diseases. Thus, individuals may later be able to buy VCEs at the pharmacy and convey the video stream from the GI tract to the phone over a wireless connection. The video footage can be preprocessed on the mobile phone too, for instance, improve the quality or do few initials analysis before the video footage is delivered to a large processing back-end. In the best instance, the first screening results are accessible within eight hours, after swallowing the VCE, which is the time taken by the camera to transverse inside the GI tract.

% Thus, the ability to execute and perform mass-screening of the GI tract relies on two fundamental research areas. First, it requires the improvement of a new generation of VCEs with better picture quality and the capacity to communicate with broadly utilized mobile phones. Second, mass-screening demands a new generation of lesion detection algorithms able to process the captured GI tract multimedia data and video footage. These multimedia data are fully automated in the mobile phone along with public cloud computing support. Here, a preliminary analysis and task-oriented compression of a captured video footage before uploading into the cloud is of great significant because of huge amount of data generated by VCEs.




%
%\begin{table*}[!t]
%\centering
%\scriptsize
%\footnotesize
%\caption{Result comparison on Kvasir-Capsule}
% TODO: extend the describe ? 
%\begin{tabular}{@{}l|l|l|l|l|l|l|l|l|l|l|l|l|l@{}}
%\toprule
%\textbf{Class:} & Normal mucosa & Reduced Mucosal View & Pylorus & Polyp & Lymphoid Hyperplasia & Ileo-Cecal valve & Hematin & Foreign Bodies & Erythematous & Erosion;  & Blood & Angiectasia & Ulcer \\ \hline

%\textbf{Count:} & 34,606 & 2399 & 1520 & 64 & 592 & 1417 & 12 & 776 & 238 & 438 & 446 & 866 & 854 \\ \hline
%\bottomrule
%\end{tabular}
%\label{tab:count}
%\end{table*}
%

%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.5\linewidth]{New_figures/dist_pie.png}
%    \caption{\textbf{The distribution of classes in Kvasir-Capsule}}
%    \label{fig:Class_count}
%\end{figure}


% \begin{equation}{\label{eq:DSC}}
% \text{F1-Score}
% =\frac{2 \times tp} {2 \times tp+ fp + fn}
% \end{equation}
% %
% \begin{equation}{\label{eq:1}}
% \text{Recall}~(Rec.) = \frac{tp} {tp+ fn}
% \end{equation}
% %
% %
% \begin{equation}{\label{eq:Prec}}
% \text{Precision}~(Prec.) =\frac{tp} {tp+ fp}
% \end{equation}
% %
% %
% \begin{equation}{\label{eq:acc}}
% \text{Accuracy}~(Acc.) =\frac{tp+ tn} {tp+ fp + tn + fn}
% \end{equation}
% %
% \begin{equation}{\label{eq:MCC}}
% \text{MCC} =\frac{tp*tn-fp*fn}{\sqrt{(tp+fp)*tp+fn)*(tn+fp)*(tn+fn)}}
% \end{equation}

% Here, tp, fp, tn, fn signifies true positives, false positives, true negatives, and false negatives, respectively. 

%

%
%
%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.5\textwidth]{New_figures/mcc_vs_through_v2.png}
%    \caption{\textbf{Comparison of MCC vs Throughput for each model}}
%    \label{fig:mccvsthrough}
%\end{figure}
%

%

%
%
%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.5\textwidth]{New_figures/mcc_vs_params_v2.png}
%    \caption{\textbf{Comparison of MCC vs parameters for each model}}
%    \label{fig:mccvsparams}
%\end{figure}


%%%%%%%%% The previous introduction section is here, consider this if you want to revert back to the previous section
\section{Introduction}
\acf{WCE} is a technology that allows gastroenterologists to visualize the small bowel (intestine). \ac{VCE} is useful for differentiating between small intestine bleeding, inflammatory bowel disease and other small bowel abnormalities~\cite{lee2019natural}. Prior to the introduction of the \ac{WCE}, physicians were not able to examine the small intestine without any surgical operation. WCE was devised by a group of researchers in Baltimore in 1989 and afterwards introduced by Given Imaging Ltd., Yoqneam, Israel, as a commercial instrument~\cite{iddan2000wireless}. The device received FDA approval for use in 2001. This capsule-shaped pill can be swallowed by the patients in the presence of clinical experts without any discomfort~\cite{suman2017detection}. Unlike conventional endoscopy procedures, this procedure investigates the small bowel without pain, sedation and air insufflation.  An additional advantage of \ac{VCE} is that it is non-invasive and easy procedure but plays a crucial role in examination and diagnosis small bowel lesions~\cite{lee2019natural}.%

%and causes less discomfort to the patient~\cite{cui2010bleeding}. %Moreover, using only standard endoscopy to regularly screen a population is impossible due to high costs, time consumption and lack of skilled medical personnel.

\begin{figure}[!t]
    \centering
    \includegraphics [width=4cm]{pill_cam.jpg}
    \caption{Olympus EC-S10 endocapsule~\cite{smedsrud2021kvasir}}.
    \label{fig:capsule}
    \vspace{-10mm}
\end{figure}

The small intestine located inside the \ac{GI} tract performs the powerful function of absorbing nutrients~\cite{meerveld2017gastrointestinal}. Ailments caused inside the small intestine can cause grave problems like growth retardation or nutrient deficiencies~\cite{meerveld2017gastrointestinal}. A major obstacle in the detection and subsequent treatment of these diseases is the anatomical location of the small intestine. While imaging of the upper \ac{GI} and large intestine is feasible with endoscopy based methods, the small intestine requires VCE. Figure~\ref{fig:capsule} shows the Olympus EC-S10 endocapsule which was used in Olympus Endocapsule 10 system~\cite{ENDOCAPSULE-10}. \ac{VCE} is performed by a small capsule equipped with a wide-angle camera. The patient consumes the capsule and the capsule traverses throughout the \ac{GI} tract and records the video which is later evaluated by a clinical expert. Given the large number of frames generated by the procedure, the subsequent analysis is monotonous and susceptible to human error which can potentially lead to a high-miss rate~\cite{kaminski2010quality}. 


\ac{CADx} systems can save significant time and resources involved in \ac{VCE} analysis. In this study, we aim to develop an automated \ac{VCE} classification algorithm that can classify \ac{VCE} frames with high accuracy and real-time speed to be used in the clinical practise. To achieve this, we propose \enquote{FocalConvNet} which integrates \ac{CNN} based modules and Focal modulation~\cite{yang2022focal} to establish a new baseline on Kvasir-Capsule~\cite{smedsrud2021kvasir}.


%We use Kvasir-Capsule~\cite{smedsrud2021kvasir}, which is a large scale VCE dataset with 13 different classes of anatomical and luminal findings categories along with classes of different aspects of mucosa and musocial lesions (pathological findings). In this paper,  Additionally, we benchmark several \ac{SOTA} \ac{CNN} and vision transformer based architectures for long tailed image classification on Kvasir-Capsule\cite{smedsrud2021kvasir}.


The main contributions of this work are summarized as follows:
\begin{enumerate}
 \item We proposed a novel deep learning architecture, named FocalConvNet, to classify anatomical and luminal findings in video frames of capsule endoscopy. We leverage the focal modulation strategy of aggregating multi-scale context for modulating the query. The focal modulation mechanism is integrated with lightweight convolutional to outperform several \ac{SOTA} image classification methods.
 
 \item FocalConvNet not only achieves the best F1-score and \ac{MCC} in classification on Kvasir-Capsule, but also its lightweight and computationally economical architecture report the highest throughput of 148 images per second.
 
 \item To advance the work on long-tailed anatomical, pathological, and mucosal view classification in \ac{VCE} frames, we provide additional comparisons with \ac{SOTA} \ac{CNN} and transformer based classification networks which otherwise lacked comparable studies.
\end{enumerate}
